A Probabilistic Modeling Approach to One-Shot Gesture Recognition

Gesture recognition enables a natural extension of the way we currently interact with devices. Commercially available gesture recognition systems are usually pre-trained and offer no option for customization by the user. In order to improve the user experience, it is desirable to allow end users to define their own gestures. This scenario requires learning from just a few training examples if we want to impose only a light training load on the user. To this end, we propose a gesture classifier based on a hierarchical probabilistic modeling approach. In this framework, high-level features that are shared among different gestures can be extracted from a large labeled data set, yielding a prior distribution for gestures. When learning new types of gestures, the learned shared prior reduces the number of required training examples for individual gestures. We implemented the proposed gesture classifier for a Myo sensor bracelet and show favorable results for the tested system on a database of 17 different gesture types. Furthermore, we propose and implement two methods to incorporate the gesture classifier in a real-time gesture recognition system.

==> figures/tikz_preamble.tex <==
% Preamble for drawing FFGs. For example:

% \begin{tikzpicture}
%     [node distance=20mm,auto,>=stealth']
%     \begin{scope}
%         %\draw[style=dotted] (0,-10cm) grid[xstep=1cm, ystep=1cm] (12cm,6cm);

%         \node[clamped] (fl) {};
%         \node[box, right of=fl, node distance=15mm] (fa) {$f_a$};
%         \node[box, right of=fa] (fb) {$f_b$};
%         \node[box, right of=fb] (fc) {$f_c$};
%         \node[clamped, right of=fc, node distance=15mm] (fr) {};
%         \node[clamped, below of=fb, node distance=15mm] (fd) {};

%         \path[line] (fl) edge[-] node[anchor=north]{$x_1$} (fa);
%         \path[line] (fa) edge[-] node[anchor=north]{$x_2$} (fb);
%         \path[line] (fb) edge[-] node[anchor=north]{$x_5$} (fc);
%         \path[line] (fc) edge[-] node[anchor=north]{$x_4$} (fr);
%         \path[line] (fb) edge[-] node[anchor=west]{$x_3$} (fd);

%         \msg{up}{right}{fa}{fb}{0.5}{1}
%         \msg{up}{right}{fb}{fc}{0.35}{2}
%         \msg{up}{left}{fb}{fc}{0.65}{3}
%     \end{scope}
% \end{tikzpicture}

\usepackage{tikz}
\usepackage{xifthen}

\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)
\definecolor{beige}{RGB}{245, 245, 220}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

\usetikzlibrary{calc, arrows, fit, positioning, patterns, decorations.pathreplacing, shapes}
\tikzstyle{dash} = [dashed, -latex,>=latex]
\tikzstyle{line} = [draw, -latex,>=latex]
\tikzstyle{smallbox} = [draw, minimum size=5.0mm, font=\scriptsize]
\tikzstyle{box} = [draw, minimum size=10.0mm]
\tikzstyle{roundbox} = [draw, circle, inner sep=0pt, minimum size=3mm]
\tikzstyle{clamped} = [draw, fill=black, minimum size=0.15cm]
\tikzstyle{msgcircle} = [shape=circle, draw, inner sep=0pt, minimum size=3.5mm, fill=white, font=\scriptsize]

% Plate notation argument order: x-left, x-right, y-top, y-bottom
\newcommand{\brackets}[4]{
      \draw[dotted, rounded corners=0.3cm, line width = 1pt] ($({#1},{#3})+(-0.3,0)$) -- ($({#1},{#3})+(-0.3,0.3)$) -- ($({#2},{#3})+(0.3,0.3)$) -- ($({#2},{#3})+(0.3,0)$);
      \draw[dotted, rounded corners=0.3cm, line width = 1pt] ($({#1},{#4})+(-0.3,0)$) -- ($({#1},{#4})+(-0.3,-0.3)$) -- ($({#2},{#4})+(0.3,-0.3)$) -- ($({#2},{#4})+(0.3,0)$);}

% Message notation argument order:
%     Circle position relative to arrow [up, down, left, right];
%     Arrow direction [up, down, left, right];
%     Start node coordinate;
%     End node coordinate
%     Position along edge;
%     Message text;
\newcommand{\msg}[6]{
      % Circle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=-5.0mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\downarrow$};
      }{}
      % Circle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{down}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=5.0mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\downarrow$};
      }{}

      % Circle down arrow right
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=-5.5mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\rightarrow$};
      }{}
      % Circle up arrow right
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{right}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=5.5mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\rightarrow$};
      }{}

      % Circle down arrow left
      \ifthenelse{\isin{#1}{down} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=-5.5mm] at (anchor) {#6};
            \node[yshift=-2.0mm] at (anchor) {$\leftarrow$};
      }{}
      % Circle up arrow left
      \ifthenelse{\isin{#1}{up} \AND \isin{#2}{left}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, yshift=5.5mm] at (anchor) {#6};
            \node[yshift=2.0mm] at (anchor) {$\leftarrow$};
      }{}

      % Circle left arrow down
      \ifthenelse{\isin{#1}{left} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=-5.0mm] at (anchor) {#6};
            \node[xshift=-1.5mm] at (anchor) {$\uparrow$};
      }{}
      % Circle right arrow down
      \ifthenelse{\isin{#1}{right} \AND \isin{#2}{up}}{
            \coordinate (anchor) at ($({#3})!{#5}!({#4})$);
            \node[msgcircle, xshift=5.0mm] at (anchor) {#6};
            \node[xshift=1.5mm] at (anchor) {$\uparrow$};
      }{}
}
